MIRA: A Multimodal Illustrated Deep Research Agent for Controllable Reports

Deep research agents are increasingly capable of searching the open web and synthesizing evidence, yet they remain poorly suited to controllable report generation in multimodal deep research. This task requires agents to handle interleaved textual and visual inputs, gather multimodal evidence through multi-step web search, and deliver comprehensive illustrated reports under user-specified requirements. Existing systems face two limitations. During reasoning, they often underuse images discovered along the search trajectory; during generation, they tend to produce fixed-form answers with limited control over report granularity, multimodal composition, and evidence grounding. We introduce MIRA, a Multimodal Illustrated Deep Research Agent for controllable reports. MIRA integrates textual and visual evidence throughout research and writing. At its core, MIRA-Harness translates user requirements into generation contracts and connects four stages: evidence collection, report submission, feedback-driven revision, and final delivery. Building on this harness, MIRA-Data constructs high-quality multi-hop multimodal research trajectories, and we post-train foundation models to operate within the workflow. Using Qwen3.6-35B-A3B, MIRA achieves state-of-the-art performance among open agents on 7 representative, established multimodal-search and deep-research-agent benchmarks, while producing user-aligned illustrated reports with traceable textual and visual evidence.

==> sections/showcase/image_heights.tex <==
\rimgheight{figures/showcase/cam/page_img_116__mcad067_fig5__6e4363d21a.jpg}{0.3000}
\rimgheight{figures/showcase/cam/page_img_117__mcad067_fig6__db4923e3f4.jpg}{0.1100}
\rimgheight{figures/showcase/concrete/concise/page_img_1__MIT-RomanConcrete-01-press__f411a2621d.jpg}{0.1920}
\rimgheight{figures/showcase/concrete/concise/page_img_21__280monteiro1-450x390__b3a7defa9f.jpg}{0.3000}
\rimgheight{figures/showcase/concrete/concise/page_img_2__MIT-RomanConcrete-press-only__beccff017f.jpg}{0.2290}
\rimgheight{figures/showcase/concrete/detail/page_img_25__MIT-cementmixing-01-press__f20c10c206.jpg}{0.2245}
\rimgheight{figures/showcase/concrete/detail/page_img_46__Ancient-Roman-Concrete-Stands-the-Test-of-Time_01__3a008da427.jpg}{0.2825}
\rimgheight{figures/showcase/concrete/detail/page_img_47__Ancient-Roman-Concrete-Stands-the-Test-of-Time_02__a1f6b12f0f.jpg}{0.3000}
\rimgheight{figures/showcase/concrete/detail/page_img_68__Briefing365_figure2-1-300x200__7e3718f071.jpg}{0.2355}
\rimgheight{figures/showcase/concrete/detail/page_img_69__Briefing365_figure3-1-300x225__f775ff8b3c.jpg}{0.2649}
\rimgheight{figures/showcase/concrete/detail/page_img_7__280monteiro1-450x390__b3a7defa9f.jpg}{0.2915}
\rimgdefer{figures/showcase/cam/page_img_240__exbotj_erv536_f0003__314ac5b4c8.jpg}


==> sections/showcase/style.tex <==
\makeatletter
\definecolor{rpaper}{RGB}{255,255,255}
\definecolor{rframe}{RGB}{176,45,58}
\definecolor{rgray}{RGB}{110,110,110}
\definecolor{rquery}{RGB}{255,242,243}

\newcommand{\rtitle}[1]{\par\noindent\parbox{\linewidth}{\raggedright\large\sffamily\bfseries\color{rframe}#1}\par\nopagebreak\vspace{4pt}}
\newcommand{\rsec}[1]{\rimg@flush\par\vspace{5pt}\noindent\parbox{\linewidth}{\raggedright\hyphenpenalty=10000\exhyphenpenalty=10000\sffamily\bfseries\color{black!85}#1}\par\nopagebreak\vspace{2pt}\nopagebreak}
\newcommand{\rsubsec}[1]{\rimg@flush\par\vspace{3pt}\noindent\parbox{\linewidth}{\raggedright\hyphenpenalty=10000\exhyphenpenalty=10000\sffamily\bfseries\small\color{rgray}#1}\par\nopagebreak\vspace{1pt}\nopagebreak}
\newcommand{\rcite}[1]{\unskip\nobreak\textsuperscript{\color{rframe}\sffamily[#1]}}
\newcommand{\rurlbreaks}{\def\UrlBreaks{\do\/\do\.\do\-\do\_\do\(\do\)\do\%\do\a\do\b\do\c\do\d\do\e
  \do\f\do\g\do\h\do\i\do\j\do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t\do\u\do\v\do\w\do\x\do\y\do\z}}
\newcommand{\rurl}[1]{\\{\scriptsize\color{rgray}\rurlbreaks\url{#1}}}
\newcommand{\rimage}[2]{\par\vspace{4pt}{\centering
  \includegraphics[width=\linewidth,height=0.20\textheight,keepaspectratio]{#1}\par
  \vspace{2pt}{\scriptsize\color{rgray}{\sffamily\bfseries\color{rframe}Image~\therimg.}\ #2\par}}\vspace{5pt}}
\newenvironment{rlist}{\begin{itemize}[beginpenalty=10000,leftmargin=12pt,itemsep=1pt,topsep=2pt,parsep=0pt]\scriptsize}{\end{itemize}}

\newenvironment{renum}{\begin{enumerate}[leftmargin=14pt,itemsep=1pt,topsep=2pt,parsep=0pt,label=\textcolor{rframe}{\sffamily\bfseries\arabic*.}]}{\end{enumerate}}

\newtcolorbox{reporthead}[2]{enhanced, colback=rquery, colframe=rframe,
  boxrule=0.6pt, arc=2pt, left=8pt, right=8pt, top=4pt, bottom=5pt,
  fonttitle=\sffamily\bfseries\small, coltitle=white,
  title={MIRA report \textperiodcentered{} #1 mode\hfill\mdseries #2}}
\newcommand{\rcardhead}{\begin{reporthead}{\rcardmode}{\rcardstats}%
  {\sffamily\bfseries\scriptsize\color{rframe}USER REQUEST}\par
  \vspace{1pt}{\footnotesize\rcardquery}\end{reporthead}\vspace{-2pt}}
\newcounter{rimg}
\newcommand{\rimgref}[1]{\,{\sffamily\bfseries\scriptsize\color{rframe}[Image~#1]}}
\newcommand{\rimgsrc}[3]{\item {\sffamily\bfseries\color{rframe}#1}\enspace #2\rurl{#3}}
\newcommand{\rimgsources}[1]{\rsubsec{Image sources}\begin{rlist}#1\end{rlist}}
\newenvironment{reportcard}[3]{%
  \begingroup\small\setlength{\parskip}{3pt plus 1pt}\setlength{\parindent}{0pt}
  \renewcommand{\emph}[1]{\textbf{##1}}
  \setlength{\columnsep}{16pt}\setlength{\columnseprule}{0.3pt}
  \renewcommand{\columnseprulecolor}{\color{rframe!40}}
  \setcounter{rimg}{0}%
  \def\rcardmode{#1}\def\rcardstats{#2}\long\def\rcardquery{#3}%
  \begin{multicols}{2}[\rcardhead][0.08\textheight]}{%
  \rimg@flush\end{multicols}\endgroup\par\vspace{10pt}}

\definecolor{tsearch}{RGB}{246,204,210}
\definecolor{tpage}{RGB}{232,140,153}
\definecolor{timage}{RGB}{190,58,80}
\definecolor{tfind}{RGB}{150,40,60}
\definecolor{tpython}{RGB}{185,183,184}
\definecolor{tsubmit}{RGB}{94,15,28}
\definecolor{tok}{RGB}{94,15,28}
\usetikzlibrary{decorations.pathreplacing}
\definecolor{tlsearch}{RGB}{246,204,210}
\definecolor{tlpage}{RGB}{232,140,153}
\definecolor{tlimage}{RGB}{190,58,80}
\definecolor{tlfind}{RGB}{150,40,60}
\definecolor{tlpython}{RGB}{185,183,184}
\definecolor{tlsubmit}{RGB}{94,15,28}
\definecolor{tlband}{RGB}{250,240,242}

\definecolor{rhl}{RGB}{238,214,215}
\newcommand{\clue}{\bgroup\markoverwith{\textcolor{rhl}{\rule[-0.55ex]{2pt}{2.45ex}}}\ULon}
\newcommand{\fact}{\bgroup\markoverwith{\lower3.5\p@\hbox{\textcolor{rframe}{\sixly\char58}}}\ULon}
\newtcolorbox{rtracebox}[1]{enhanced, colback=rhl!40, colframe=rframe!70,
  boxrule=0pt, leftrule=2.2pt, arc=0pt, left=4pt, right=4pt, top=2pt, bottom=2pt,
  before skip=4pt plus 1pt, after skip=3pt plus 1pt, fontupper=\sffamily\scriptsize,
  before upper={{\bfseries\color{rframe}TRACE}\ \ #1\par\vspace{1pt}}}
\newsavebox\rtr@box
\newcommand{\rtrace}[2]{\rimg@flush\par\global\setbox\rtr@box\vbox{\hsize\linewidth\begin{rtracebox}{#1}#2\end{rtracebox}}}
\newtcolorbox{rnotebox}{enhanced, colback=white, colframe=rframe!70, boxrule=0.5pt,
  borderline={0.5pt}{0pt}{rframe!70, dashed}, frame hidden, arc=2pt,
  left=4pt, right=4pt, top=2pt, bottom=2pt, before skip=3pt plus 1pt, after skip=4pt plus 1pt,
  fontupper=\sffamily\scriptsize,
  before upper={{\bfseries\color{rframe}NOTE}\ \ }}
\newcommand{\rnote}[1]{\rimg@flush\begin{rnotebox}#1\end{rnotebox}}
\newcommand{\rbox}[5]{\draw[rframe, line width=1.1pt, rounded corners=1.5pt] (#1,#2) rectangle (#3,#4);
  \if\relax\detokenize{#5}\relax\else
  \node[anchor=south west, inner sep=1.5pt, fill=rframe, text=white, font=\sffamily\bfseries\tiny,
    rounded corners=1pt] at (#1,#4) {#5};\fi}
\newcommand{\rimgheight}[2]{\@namedef{rimgh@#1}{#2}}
\newwrite\rimg@out\immediate\openout\rimg@out=\jobname.rimg
\newsavebox\rimg@box
\newcommand{\rimgdefer}[1]{\@namedef{rimgd@#1}{}}
\newsavebox\rimg@held
\newcommand{\rimg@flush}{\ifvoid\rimg@held\else\par\unvbox\rimg@held\global\setbox\rimg@held\box\voidb@x\par\fi}
\newcommand{\rimagebox}[3]{\par\refstepcounter{rimg}%
  \edef\rimg@h{\ifcsname rimgh@#1\endcsname\csname rimgh@#1\endcsname\else 0.20\fi}%
  \sbox\rimg@box{\includegraphics[width=\linewidth,height=\rimg@h\textheight,keepaspectratio]{#1}}%
  \setbox0\vbox{\hsize\linewidth
  \ifvoid\rtr@box\else\unvbox\rtr@box\global\setbox\rtr@box\box\voidb@x\par\fi
  \vspace{2pt plus 1pt}%
  \noindent\parbox{\linewidth}{\centering
  \pdfsavepos\edef\rimg@w{\write\rimg@out{#1 \noexpand\thepage\space\noexpand\the\noexpand\pdflastxpos
    \space\noexpand\the\noexpand\pdflastypos\space\the\wd\rimg@box\space\the\ht\rimg@box\space\rimg@h
    \ifcsname rimgd@#1\endcsname\space D\fi}}\rimg@w
  \begin{tikzpicture}
  \node[inner sep=0pt, anchor=south west] (img) {\usebox\rimg@box};
  \begin{scope}[x={(img.south east)}, y={(img.north west)}]#3\end{scope}
  \end{tikzpicture}\par
  \vspace{2pt}{\scriptsize\color{rgray}{\sffamily\bfseries\color{rframe}Image~\therimg.}\ #2\par}}\par\vspace{5pt plus 1pt}}%
  \ifcsname rimgd@#1\endcsname
    \global\setbox\rimg@held\vbox{\ifvoid\rimg@held\else\unvbox\rimg@held\fi\unvbox0}%
  \else \rimg@flush\unvbox0\par\fi}
\input{sections/showcase/image_heights}
\newtcolorbox{rgatebox}{enhanced, colback=black!3, colframe=black!35, boxrule=0.4pt, arc=2pt,
  left=5pt, right=5pt, top=3pt, bottom=3pt, before skip=6pt, fontupper=\sffamily\scriptsize,
  before upper={{\bfseries\color{rframe}REPORT GATE RECORD}\par\vspace{1pt}}}
\newcommand{\rgate}[1]{\rimg@flush\begin{rgatebox}\begin{itemize}[leftmargin=10pt,itemsep=0pt,topsep=1pt,parsep=0pt]#1\end{itemize}\end{rgatebox}}

\definecolor{radd}{RGB}{255,214,219}
\newcommand{\dadd}{\bgroup\markoverwith{\textcolor{radd}{\rule[-0.55ex]{2pt}{2.45ex}}}\ULon}
\newcommand{\cmprow}[3]{\raggedright{\sffamily\bfseries\scriptsize\color{rframe}#1} & \raggedright #2 & \raggedright #3 \tabularnewline \midrule}
\newcommand{\cmpnone}{{\color{black!40}not covered}}
\newenvironment{rlegendbox}{\par
  \ifdim\dimexpr\pagegoal-\pagetotal\relax<0.06\textheight\newpage\fi
  \vspace{6pt}\noindent{\color{rframe}\rule{\linewidth}{0.6pt}}\par
  \nopagebreak\vspace{1pt}{\sffamily\bfseries\scriptsize\color{rframe}HOW TO READ THE ANNOTATED REPORTS}\par
  \nopagebreak\vspace{1pt}\begingroup\sffamily\scriptsize\setlength{\parindent}{0pt}}{%
  \par\endgroup\vspace{1pt}\noindent{\color{rframe}\rule{\linewidth}{0.6pt}}\par\vspace{8pt}}
\makeatother

